Approximate Minimum Diameter

We study the minimum diameter problem for a set of inexact points. By inexact, we mean that the precise location of the points is not known. Instead, the location of each point is restricted to a contineus region ($\impre$ model) or a finite set of points ($\indec$ model). Given a set of inexact points in one of $\impre$ or $\indec$ models, we wish to provide a lower-bound on the diameter of the real points. In the first part of the paper, we focus on $\indec$ model. We present an $O(2^{\frac{1}{\epsilon^d}} \cdot \epsilon^{-2d} \cdot n^3 )$ time approximation algorithm of factor $(1+\epsilon)$ for finding minimum diameter of a set of points in $d$ dimensions. This improves the previously proposed algorithms for this problem substantially. Next, we consider the problem in $\impre$ model. In $d$-dimensional space, we propose a polynomial time $\sqrt{d}$-approximation algorithm. In addition, for $d=2$, we define the notion of $\alpha$-separability and use our algorithm for $\indec$ model to obtain $(1+\epsilon)$-approximation algorithm for a set of $\alpha$-separable regions in time $O(2^{\frac{1}{\epsilon^2}}\allowbreak . \frac{n^3}{\epsilon^{10} .\sin(\alpha/2)^3} )$.

==> sections/ApproxMinDiameterImprecise.tex <==
\section{Approximation algorithm for $\pt$\label{sec-apxmindim2}}

In this section, we consider the problem of finding minimum diameter in $\impre$ model. As mentioned, in this model an imprecise point is represented by a continues region. Given a set ${\cal R} = \{{\cal R}_1, {\cal R}_2, \ldots, {\cal R}_n\}$ where each ${\cal R}_i$ is a polygonal region. A \textbf{selection} $S=\{s_1, s_2, ..., s_n\}$ of ${\cal R}$ is a set of points where $s_i \in {\cal R}_i$. In the minimum diameter problem, the goal is to find a selection $S$ such that $D(S)$ is minimized among all options. 
We consider the problem for the case where every ${\cal R}_i$ is a polygonal convex region with constant complexity (i.e., number of edges).


In Section \ref{sqrty}, we present a polynomial time $\sqrt{d}$-approximation algorithm for $\pt$. 

\subsection{$\sqrt{d}$-approximation} \label{sqrty}
Our $\sqrt{d}$-approximation construction is based on $LP$-programming which uses the rectilinear distances ($d_{l_1}$) of the points. For now, suppose that $d$ is constant and consider $LP$~\ref{LP1}. In this $LP$, we want to select the points $s_1,s_2,\ldots,s_n$ such that $s_i \in {\cal R}_i$ and the rectilinear diameter of these points is minimized. 

\begin{equation}
\label{LP1}
\begin{array}{ll@{}ll}
\textbf{LP~\ref{LP1}:}  & &\\
\text{minimize}  &\quad \displaystyle  \ell &\\
\text{subject to}&\quad \displaystyle d_{l_1}(s_i, \ s_j)   &\leq \ell  &\quad\forall i,j\\
                 &                       \quad\qquad\qquad                         s_{i} &\in {\cal R}_i &\quad\forall i,j
\end{array}
\end{equation}


We show that $d_{l_1}(s_i,s_j)$ can be expressed by $2^d$ linear constraints (note that $ d_{l_1}(s_i,s_j) = |s_{i,1}-s_{j,1}| + \ldots + |s_{i,d}-s_{j,d}|$). Based on the relative value of $s_{i,k}, s_{j,k}$, there are $2^d$ different possible expressions for $d_{l_1}(s_i,s_j)$. For example, for $d=2$, we have:

\[
 d_{l_1}(s_i, \ s_j) =
  \begin{cases}
  s_{i,1} - s_{j,1} + s_{i,2} - s_{j,2} &\qquad  s_{i,1} \ge s_{j,1} \qquad s_{i,2} \ge s_{j,2}\\
  
  s_{j,1} - s_{i,1} + s_{i,2} - s_{j,2} &\qquad  s_{i,1} < s_{j,1} \qquad s_{i,2} \ge s_{j,2}\\
    
  s_{i,1} - s_{j,1} + s_{j,2} - s_{i,2} &\qquad  s_{i,1} \ge s_{j,1} \qquad s_{i,2} < s_{j,2} \\
  
  s_{j,1} - s_{i,1} + s_{j,2} - s_{i,2} &\qquad  s_{i,1} < s_{j,1} \qquad s_{i,2} < s_{j,2} \\

  \end{cases}
\]

Call these expressions as $e_1,e_2,\ldots,e_{2^d}$. Note that if $d_{l_1}(s_i, \ s_j) \leq \ell$, then for all $1 \le k \le 2^n$, $e_k \le \ell$. With this in mind, we can replace $d_{l_1}(s_i, \ s_j) \leq \ell$ with these $2^d$ linear expressions. It is worth mentioning that we can reduce the number of expressions of this type in $LP$~\ref{LP1} using some additional variables, see Section \ref{const} for more details.


Since the regions are convex, the constraint $s_i \in {\cal R}_i$ can be described by $|{\cal R}_i|$ linear inequalities where $|{\cal R}_i|$ is the complexity of region ${\cal R}_i$. Thus, the number of the constraints of this type is $|{\cal R}| = \sum_i |{\cal R}_i|$. Therefore, total number of the constraints would be $2^d \cdot n^2 + |{\cal R}|$ which is $\textsf{poly}(n)$ for constant $d$. 

\begin{theorem}
\label{t2}
$D_{min} \leq \ell \leq \sqrt{d}D_{min}$.
\end{theorem}

\begin{proof}
Let $S_{min}$ be the optimal selection of $R$ so that $D_{min} = D(S_{min})$. Obviously, $\ell \ge D_{min}$. On the other hand, $S_{min}$ is a feasible solution for $LP$~\ref{LP1} with rectilinear diameter at most $\sqrt{d} D_{min}$. 
\end{proof}

Theorem~\ref{t2} shows that $LP$~\ref{LP1} results in a $\sqrt{d}$ approximation algorithm for $\pt$. We use this result to bound the optimal solution in Section \ref{epsax}.


\input{sections/appendix.tex}





\subsection{$(1+\epsilon)$-approximation for $d=2$}\label{epsax}
In this section, we propose an $\epsilon$-approximation algorithm for $\pt$ when $d=2$ and the regions in ${\cal R}$ admit a special notion of separability, called $\alpha $-separability.

\subsubsection{$\alpha$-separability}
\begin{definition}
Two intersecting lines, divide the plane into four areas. Two regions $A$ and $B$ are separated by these lines, if they completely belong to opposite areas, See Fig.~\ref{fig:sep}(a). In Fig.~\ref{fig:sep}(a), we name $\alpha$ as the degree of separation.

%\begin{figure}
%\centering
%\includegraphics[scale = 0.8]{epsANDspecial}
%\caption{(a) Regions are separated by two intersecting lines. Also the optimal solution $S_{min}$, must be entirely within the rectangle $XYZT$. (b) Special cases.}
%\label{fig:separability}
%\end{figure}
%\end{definition}
%\begin{definition}
%Two regions $X$ and $Y$ are $\alpha$-separable, if there exists two intersecting lines  separating them, with degree of separation equals to $\alpha$.


\begin{figure}[t!]
  \centering
  \includegraphics[width=1.0\linewidth]{eps1va2}   
  \caption{(a) Regions are separated by two intersecting lines. The optimal solution $S_{min}$, must be entirely within the rectangle $XYZT$. (b) The points inside the green area are at least $R$ distance away from the region $A$ (similar fact is intact between the points inside the blue area and the region $B$).}
  \label{fig:sep}
\end{figure}


% \begin{figure}
% \centering
% \includegraphics[scale=0.6]{eps}
% \caption{Regions are separated by two intersecting lines. Also the optimal solution $S_{min}$, must be entirely within the rectangle $XYZT$.}
% \label{fig:separability}
% \end{figure}

\end{definition}


\begin{definition}
A set $S$ of regions is $\alpha$-separable, if \textbf{there exists} two regions $X$ and $Y$ in $S$, which are $\alpha$-separable.
\end{definition}

\begin{definition}
For two regions $X$ and $Y$, maximum degree of separability is defined as the maximum $\alpha$, such that $X$ and $Y$ are $\alpha$-separable. Subsequently, maximum degree of separability for a set $\cal R$ of regions, is the maximum possible $\alpha$, such that $\cal R$ is $\alpha$-separable.

\end{definition} 

It's easy to observe that the maximum degree of separability for two regions  can be computed in polynomial time by computing the common tangent of the regions. Similarly, maximum degree of separability for a set $\cal R$ of regions, can be computed in polynomial time.


Note that the maximum degree of separability is not well defined for the case, where every pair of regions have a nonempty intersection. We postpone resolving this issue to Section~\ref{aDiscussion}. For now, we suppose that ${\cal R}$ contains at least two regions that are completely disjoint.

\subsubsection{$(1+ \epsilon)$-approximation algorithm}


\begin{theorem}
Let $\cal R$ be an $\alpha$-separable set of regions. then there exists an $\epsilon$-approximation algorithm for computing $\pt$ of $\cal R$ with running time $O(2^{\frac{1}{\epsilon^2}}\allowbreak . \frac{n^3}{\epsilon^{10} .\sin(\alpha/2)^3} )$.
\end{theorem}
\begin{proof}
Assume that $A,B$ are the regions in ${\cal R}$, that are $\alpha$-separable. Fig.~\ref{fig:sep}(a) shows the regions and the separating lines. Let $R$ be the value, with the property that $D_{min} \le R \le \sqrt{2}D_{min}$. Such $R$ can be computed by the  $\sqrt{d}$-approximation algorithm described in section 3.1.

Argue that the points in the optimal solution $S_{min}$ must be entirely within the rectangle $XYZT$ (See Fig.~\ref{fig:sep}(a)), while every point out of the rectangle has distance more than $R$ to at least one of the selected points from regions $A$ or $B$ (see Fig.~\ref{fig:sep}(b)). The area of $XYZT$ is $\frac{4R^2}{\sin(\alpha/2)}$, that is, $O(\frac{R^2}{\sin(\alpha/2)})$.


% \begin{figure}
% \centering
% \includegraphics[scale=0.4]{eps2}
% \caption{Any point out of $XYZT$ has a distance more than $R$ to at least one of $A$ or $B$}
% \label{fig:separability2}
% \end{figure}

Color each region $R_i$ with color $c_i$. Now, construct a grid $\mathbb{G}$ on the rectangle $XYZT$ with cells of size $\epsilon R$.
For each grid point $p$ and region $R_i$ containing $p$ create a point with the same location as $p$ and color $c_i$, see Fig.~\ref{fig:gridVesp}(a). Total number of the points is $O(\frac{n}{\epsilon^2 \sin(\alpha/2)})$.


\begin{figure}[t!]
  \centering
  \includegraphics[width=1.0\linewidth]{eps3ANDespecial}   
  \caption{(a) Constructing a grid on $XYZT$. (b) Special cases.}
  \label{fig:gridVesp}
\end{figure}

% \begin{figure}
% \centering
% \includegraphics[scale=0.6]{eps3}
% \caption{Constructing a grid on $XYZT$}
% \label{fig:separability3}
% \end{figure}
 
 
Let $P$ be the set of generated points. We give $P$ as an input instance for $\md$ problem. Next, using algorithm~\ref{alg:packed-dna-hamming} we find a color selection $Q$ with $D(Q) \leq (1+\epsilon)D_{min}$ where $D_{min}$ is the diameter of the optimal selection. While the diameter of each cell in $\mathbb{G}$ equals $\sqrt{2} \epsilon = O(\epsilon)$, total error of selection $Q$ for $\pt$ is $O(\epsilon)$.
Considering the time complexity obtained for $\md$, total running time would be $O(2^{\frac{1}{\epsilon^2}}\allowbreak . \frac{n^3}{\epsilon^{10} \cdot \sin{(\alpha/2)}^3} )$. 


\end{proof}

Note that $1 / \sin (\alpha)$ is exponentially descending for $0 \leq \alpha  \leq \pi/2$. As an example, for $\alpha > 20^{\circ}$,  $1 / \sin (\alpha) < 3$ and for $\alpha>45^{\circ}$, $1 / \sin (\alpha) < 1.5$. Thus, 
for large enough $\alpha$ (e.g. $\alpha>10$), we can consider this value as a constant. 


\subsection{A discussion on $\alpha$-separability}\label{aDiscussion}
As previously mentioned, $\alpha$-separability is not well defined in the case that all pairs of the regions have a nonempty intersection. In this section, we wish to address this issue. 

Note that by \textbf{Helly's theorem}, if every triple regions of the set ${\cal R}$ have a nonempty intersection, then the intersection of all the regions
in ${\cal R}$ is nonempty, i.e., $ \bigcap_i {\cal R}_i \neq \emptyset.$ In this case, the optimal selection in $\pt$ is trivial: select the same point for all the regions.
Thus, we can assume that there exists a set of three regions, namely, $A,B,$ and $C$ in ${\cal R}$ such that any pair of them has a nonempty intersection, but $A \cap B \cap C$ is empty. 

Denote by $p_A, p_B,$ and $p_C$ the selected points from the regions $A, B,$ and $C$, respectively. To solve the problem of $\md$ on ${\cal R}$ we divide the problem into three sub problems: $(i)$ $\{p_A,p_B\} \in A \cap B$, $(ii)$ $p_A \in (A \setminus B)$ and $p_B \in (B \setminus A)$, and $(iii)$ $p_A \in A \cap B$ and $p_B \in (A \setminus B)$.


% \begin{figure}
% \centering
% \includegraphics[scale = 0.6]{special}
% \caption{Special Cases}
% \label{fig:special}
% \end{figure}


For the first case, we can assume w.l.o.g that $p_A$ and $p_B$ are in the same location in $A \cap B$. Thus, we can remove $A \Delta B$ and only keep $A \cap B$. Since the intersection of $(A \cap B)$ and $C$  is empty, they are separable.

For the second case, we partition $A \Delta B$ into the constant number of convex sub-regions (for example, by triangulating $A \Delta B$ as shown in Fig.~\ref{fig:gridVesp}(b)). Suppose that $A \setminus B$ is divided into $r$ sub-regions and $B \setminus A$ is divided into $s$ sub-regions. Then we solve $r \times s$ sub-problems, according to the sub-regions $p_A$ and $p_B$ belong. In all of these sub-problems, $\alpha$-separability is well defined.

Finally, note that considering the third case is not necessary, since if $p_A \in A \cap B$ and $p_B \notin A \cap B$ then we can move $p_B$ to the same location as $p_A$ without any decrease in the diameter of the selected points.




==> thebibliography.tex <==

\bibitem{aggarwal2009trio}
Aggarwal, Charu C. "Trio a system for data uncertainty and lineage." Managing and Mining Uncertain Data. Springer US, 2009. 1-35.

\bibite{cormode2009semantics}
Cormode, Graham, Feifei Li, and Ke Yi. "Semantics of ranking queries for probabilistic data and expected ranks." Data Engineering, 2009. ICDE'09. IEEE 25th International Conference on. IEEE, 2009.

\bibitem{jorgensen2011geometric}
J{\o}rgensen, Allan and L{\"o}ffler, Maarten and Phillips, Jeff M, Geometric computations on indecisive points,
  Algorithms and Data Structures, Berlin Heidelberg, 2011. 536-547.

\bibitem{fan2013expected}
Fan, Chenglin and Luo, Jun and Zhong, Farong and Zhu, Binhai, Expected Computations on Color Spanning Sets,
  Frontiers in Algorithmics and Algorithmic Aspects in Information and Management, Springer (2013) 130--141.


\bibitem{fleischer2011computing}
R.~Fleischer, X.~Xu, Computing minimum diameter color-spanning sets is hard,
  Information Processing Letters 111~(21) (2011) 1054--1056.

\bibitem{fleischer2010computing}
R.~Fleischer, X.~Xu, Computing minimum diameter color-spanning sets, in:
  Frontiers in Algorithmics, Springer, 2010, pp. 285--292.

\bibitem{zhang2009keyword}
D.~Zhang, Y.~M. Chee, A.~Mondal, A.~Tung, M.~Kitsuregawa, Keyword search in
  spatial databases: Towards searching by document, in: Data Engineering, 2009.
  ICDE'09. IEEE 25th International Conference on, IEEE, 2009, pp. 688--699.

\bibitem{fan2011some}
W.~Ju, C.~Fan, J.~Luo, B.~Zhu, O.~Daescu, On some geometric problems of
  color-spanning sets, Journal of Combinatorial Optimization 26~(2) (2013)
  266--283.

\bibitem{consuegrageometric}
M.~E. Consuegra, G.~Narasimhan, S.-i. Tanigawa, Geometric avatar problems, in:
  IARCS Annual Conference on Foundations of Software Technology and Theoretical
  Computer Science (FSTTCS 2013), Vol.~24, Schloss Dagstuhl--Leibniz-Zentrum
  fuer Informatik, 2013, pp. 389--400.

\bibitem{agarwal2004approximating}
P.~K. Agarwal, S.~Har-Peled, K.~R. Varadarajan, Approximating extent measures
  of points, Journal of the ACM (JACM) 51~(4) (2004) 606--635.

\bibitem{loffler2010largest}
M.~L{\"o}ffler, M.~van Kreveld, Largest bounding box, smallest diameter, and
  related problems on imprecise points, Computational Geometry 43~(4) (2010)
  419--433.

\bibitem{zarrabi2008geometric}
H.~Zarrabi-Zadeh, Geometric approximation algorithms in the online and data
  stream models, Ph.D. thesis, University of Waterloo (2008).

\bibitem{sariel2011geometric}
S.~Har-Peled, Geometric approximation algorithms, no. 173, American
  Mathematical Soc., 2011.

\bibitem{kruger2008basic}
H.~Kruger, Basic measures for imprecise point sets in rd, Master's thesis,
  Utrecht University.
